Digital Modeling for Everyone: Exploring How Novices Approach Voice-Based 3D Modeling

Manufacturing tools like 3D printers have become accessible to the wider society, making the promise of digital fabrication for everyone seemingly reachable. While the actual manufacturing process is largely automated today, users still require knowledge of complex design applications to produce ready-designed objects and adapt them to their needs or design new objects from scratch. To lower the barrier to the design and customization of personalized 3D models, we explored novice mental models in voice-based 3D modeling by conducting a high-fidelity Wizard of Oz study with 22 participants. We performed a thematic analysis of the collected data to understand how the mental model of novices translates into voice-based 3D modeling. We conclude with design implications for voice assistants. For example, they have to: deal with vague, incomplete and wrong commands; provide a set of straightforward commands to shape simple and composite objects; and offer different strategies to select 3D objects.

==> meta/copyright.tex <==
\setcopyright{acmlicensed}
\copyrightyear{2023}
\acmYear{2023}
\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
\acmConference[Submitted to CHI '23]{Submitted to CHI Conference on Human Factors in Computing Systems}{April 30 -- May 6, 2023}{Hamburg, Germany}
\acmBooktitle{Submitted to CHI Conference on Human Factors in Computing Systems (CHI '23), April 30 -- May 6, 2023, Hamburg, Germany}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}

==> meta/definitions.tex <==
\newcommand{\systemname}{}
% \newcommand{\longtitle}{Designing Truly Conversational Agents for 3D-modeling: Requirements and Challenges}
\newcommand{\longtitle}{Digital Modeling for Everyone: Exploring How Novices Approach Voice-Based 3D Design}

% We need a short title for the running headers
\title[Digital Modeling for Everyone]{\longtitle{}}


\newcommand{\cmissing}{\todo{[citation missing]}}

% CANDIDATE TITLES:
% [AE] Reducing the Cost of Entry of Digital Fabrication: Requirements and Challenges of Designing a Voice-Based 3D Modelling System
% [AE] Democratizing Digital Fabrication: Requirements and Challenges of Designing a Voice-Based 3D Modelling System
% [AE] Towards the Democratization of Digital Fabrication: Requirements and Challenges of Designing a Voice-Based 3D Modelling System
% [AE] Towards the Democratization of Digital Fabrication: Symplifying 3D Modelling Systems through Voice Interaction
% [AE] Democratizing Digital Fabrication: Exploring Novices' Approaches to Voice-Based 3D Modelling
% (++) [AE] Democratizing Digital Fabrication: Exploring how Novices Approach Voice-Based 3D Modelling
% [AE] From Thought to Model: Democratizing Digital Fabrication Through Voice-Based Interaction
% (+) [GD] Democratizing Digital Fabrication: explore how the mental model of non-experts translate into voice-based 3D modeling




==> meta/meta.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10003120.10003121.10003124.10010870</concept_id>
       <concept_desc>Human-centered computing~Natural language interfaces</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10003120.10003121.10003122.10003334</concept_id>
       <concept_desc>Human-centered computing~User studies</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010405.10010481.10010483</concept_id>
       <concept_desc>Applied computing~Computer-aided manufacturing</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Natural language interfaces}
\ccsdesc[500]{Human-centered computing~User studies}
\ccsdesc[300]{Applied computing~Computer-aided manufacturing}
%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Digital Fabrication, 3D Design, Voice Interaction, Wizard of Oz Study}

==> meta/stats.tex <==
\newcommand{\anovaCor}[6]{$F_{#1, #2}=#3$, $p#4$, $\epsilon=#5$\subEtaG{#4}{#6}}
\newcommand{\anova}[5]{$F_{#1, #2}=#3$, $p#4$\subEtaG{#4}{#5}}
\newcommand{\anovaCorWithoutEffect}[5]{$F_{#1, #2}=#3$, $p#4$, $\epsilon=#5$}
\newcommand{\anovaWithoutEffect}[4]{$F_{#1, #2}=#3$, $p#4$}


\newcommand{\subEtaG}[2]{%
	\ifthenelse{\equal{#1}{\string >.05}}
	{}
	{, $\eta_{G}^{2}=#2$}%
}

\newcommand{\subEta}[2]{%
	\ifthenelse{\equal{#1}{\string >.05}}
	{}
	{, $\eta^{2}=#2$}%
}

\newcommand{\friedman}[3]{$\chi^2(#1) = #2$, $p #3$}

\newcommand{\srh}[3]{$\chi^2(#1) = #2$, $p #3$}

\newcommand{\valSi}[3]{$\mu = \SI[round-mode=places,round-precision=1]{#1}{#3}$, $\sigma = \SI[round-mode=places,round-precision=1]{#2}{#3}$}
\newcommand{\val}[2]{$\mu = \num[round-mode=places,round-precision=1]{#1}$, $\sigma = \num[round-mode=places,round-precision=1]{#2}$}
\newcommand{\se}[1]{$\sigma_{\overline{x}} = #1$}

\newcommand{\emm}[2]{\ac{EMM} $\mu = #1$, \se{#2}}
\newcommand{\emmSi}[3]{\ac{EMM} $\mu = \SI{#1}{#3}$, \se{\SI{#2}{#3}}}
%{5.89}{0.37}{5.12}{6.65}
%\newcommand{\emmCI}[5]{\ac{EMM} $\mu = \SI{#1 #5}$ [\SI{#3 #5},\SI{#4 #5}]}
%\newcommand{\emmCI}[4]{$\mu = #1$ [#3,#4]}

\newcommand{\muemm}{\mu_{\scriptscriptstyle EMM}}

%\newcommand{\emmCI}[5]{$\ac{EMM}~\mu~=~#1#5$ [#3#5,#4#5]}
\newcommand{\emmCI}[5]{$\muemm{}~=~\num[round-mode=places,round-precision=1]{#1}#5$ [\num[round-mode=places,round-precision=1]{#3}#5, \num[round-mode=places,round-precision=1]{#4}#5]}

\newcommand{\emmP}[2]{\emm{#1\%}{#2\%}}
\newcommand{\valP}[2]{\val{#1\%}{#2\%}}

\newcommand{\pearson}[2]{$r = #1$, $p#2$}

\def\gge{$\epsilon$}
\def\petasquared{$\eta_{p}^{2}$}
\def\etasquared{$\eta_{}^{2}$}
\def\ges{$\eta_{G}^{2}$}


